Hyper-reduction for Petrov-Galerkin reduced order models

Projection-based Reduced Order Models minimize the discrete residual of a "full order model" (FOM) while constraining the unknowns to a reduced dimension space. For problems with symmetric positive definite (SPD) Jacobians, this is optimally achieved by projecting the full order residual onto the approximation basis (Galerkin Projection). This is sub-optimal for non-SPD Jacobians as it only minimizes the projection of the residual, not the residual itself. An alternative is to directly minimize the 2-norm of the residual, achievable using QR factorization or the method of the normal equations (LSPG). The first approach involves constructing and factorizing a large matrix, while LSPG avoids this but requires constructing a product element by element, necessitating a complementary mesh and adding complexity to the hyper-reduction process. This work proposes an alternative based on Petrov-Galerkin minimization. We choose a left basis for a least-squares minimization on a reduced problem, ensuring the discrete full order residual is minimized. This is applicable to both SPD and non-SPD Jacobians, allowing element-by-element assembly, avoiding the use of a complementary mesh, and simplifying finite element implementation. The technique is suitable for hyper-reduction using the Empirical Cubature Method and is applicable in nonlinear reduction procedures.

==> Hyper_reduction.tex <==
\section{Hyper-reduction}
\subsection{Galerkin-based ROMs}
\label{Galerkin-based ROMs}
To address the issue of hyper-reduction in the context
of the least-squares formulation, it is better first to revistit the standard HROM in Galerkin projections \cite{Everson1995,Chaturantabut2010,Farhat2015,Joaquin2016,Joaquin2020}, where the reduced-order equation to be solved for marching the solution from $t_n$ to $t_{n+1}$ is of the form:
\begin{equation}
    \mathbf{\Phi}^T\mathbf{R}(\mathbf{u}_n+\mathbf{\Phi} \mathbf{\Delta q};\boldsymbol{\mu})=\mathbf{0}
    \label{Galerkin projected residual}
\end{equation}
In terms of the assembly of elemental contributions, the expression above adopts the following form:
\begin{equation}
    \mathbf{\Phi}^T\mathbf{R}=\mathbf{\Phi}^T\sum_{e=1}^{M}\mathbf{L}^{e^T}\mathbf{R}^{e}=\sum_{e=1}^{M}(\mathbf{L}^{e}\mathbf{\Phi})^T\mathbf{R}^{e}=\sum_{e=1}^{M}\mathbf{\Phi}^{e^T}\mathbf{R}^{e}=\mathbf{0}
    \label{Galerkin assembly of elemental contributions}
\end{equation}
terms were defined in \ref{FOM Assembly} . This equation shows that, despite the fact that $n<< N$ (the equation solving effort has drastically diminished), the computational complexity of the problem still scales with the size of the discretization of the underlying finite elements (considering that it is necessary to loop over the $M$ finite elements of the mesh to assemble the residual and thereby the Jacobian matrices).\\
\\
The hyper-reduction scheme allows us to replace eq.\ref{Galerkin assembly of elemental contributions} by an approximated version of the form:
\begin{equation}
    \sum_{e\in \mathbf{Z}}w^e\mathbf{\Phi}^{e^T}\mathbf{R}^e=\mathbf{0}
\end{equation}
Here $\mathbf{Z}\subset \{1,2,\hdots,M\}$ is a subset of finite elements of cardinality $m$, whereas $w^e\in \mathbb{R}_{+}(e=1,2,\hdots, m)$ are positive weights of the a set $\mathbf{W}\in\mathbb{R}^m$.\\
In the current work, we use the ``\textit{Empirical Cubature Method}" (ECM) proposed in  \cite{Joaquin2016}, and later refined in \cite{Joaquin2020} to arrive at the set of reduced elements and weights.
\\
\\
The essential idea of such method is to solve eq.\ref{Galerkin assembly of elemental contributions} for the same input parameters employed in the first reduction stage. Next, the reduced equation is expressed in a matrix format as follows:
\begin{equation}
    \sum_{e=1}^M\mathbf{\Phi}^{e^T}\mathbf{R}_i^e=
    \begin{bmatrix}
    \mathbf{\Phi}^{1^T}\mathbf{R}_i^1, & \mathbf{\Phi}^{2^T}\mathbf{R}_i^2, & \hdots, & \mathbf{\Phi}^{M^T}\mathbf{R}_i^M
    \end{bmatrix}\mathcal{I}=\mathbf{0},
    \qquad \qquad \qquad
    i=1,2,\hdots,P
    \label{Projected Residuals}
\end{equation}
where:
\begin{equation}
    \mathcal{I}:=
    \begin{bmatrix}
    1\\
    1\\
    \vdots\\
    1
    \end{bmatrix}
\end{equation}
Let us construct a matrix $\mathbf{A}\in \mathbb{R}^{P\times M}$ formed by collecting the block column matrix from eq.\ref{Projected Residuals} for all training parameters.
\begin{equation}
    \mathbf{A}^{(\mathbf{\Phi})}=
    \begin{bmatrix}
    \mathbf{A}_1^{(\mathbf{\Phi})},&\mathbf{A}_2^{(\mathbf{\Phi})},&\hdots&\mathbf{A}_M^{(\mathbf{\Phi})}
    \end{bmatrix}
\end{equation}
where each block column $\mathbf{A}_e\in \mathbb{R}^{P}$ is given by:
\begin{equation}
    \mathbf{A}_e^{(\mathbf{\Phi})}=
    \begin{bmatrix}
    \mathbf{\Phi}^{e^T}\mathbf{R}^e(\boldsymbol{\mu}_1)\\
    \mathbf{\Phi}^{e^T}\mathbf{R}^e(\boldsymbol{\mu}_2)\\
    \vdots\\
    \mathbf{\Phi}^{e^T}\mathbf{R}^e(\boldsymbol{\mu}_P)\\
    \end{bmatrix}
\end{equation}
Keep in mind that this matrix meets the condition $\mathbf{A}^{(\mathbf{\Phi})}\mathcal{I}=\mathbf{0}$.
Let $m-1$ be the numeric rank of $\mathbf{A}^{(\mathbf{\Phi})}$, determined by a user-prescribed tolerance $0\leq\epsilon < 1$. Then, it is shown in \cite{Joaquin2016} that there is at least one set of elements $\mathbf{Z}\subset \{1,2,\hdots,M\}$ and positive weights $\mathbf{W}\in \mathbb{R}^m$ such that:
\begin{equation}
    \|\mathbf{A}^{(\mathbf{\Phi})}\mathcal{I}\|_2^2\approx \|\mathbf{A}_\mathbf{Z}^{(\mathbf{\Phi})}\mathbf{W}\|_2^2=\mathcal{O}(\epsilon)
\end{equation}
where $\mathbf{A}_Z^{(\mathbf{\Phi})}$ is the block matrix of $\mathbf{A}^{(\mathbf{\Phi})}$ formed by the columns corresponding to the indexes $\mathbf{Z}$, whereas $\mathbf{W}=[w^1,w^2,\hdots,w^m]^T$. The reader is referred to \cite{Joaquin2020} for details on the algorithm that enables one to select the elements $\mathbf{Z}$ and the weights $\mathbf{W}$. \\
We remark that the hyperreduction approximation does not attempt to accurately represent the high-dimensional residual (FOM), but only its projection onto the left subspace spanned by the columns of the left reduced order basis (ROM).
\subsection{Extension to least-squares problems}
For the sake of simplicity, let us focus on the case $\mathbf{G}=\mathbf{I}$, i.e., when the minimization is carried out in the 2-norm; in this case, eq.\ref{Minimization of the residual} becomes:
\begin{equation}
    \mathbf{\Phi}^T\mathbf{K}^T(\mathbf{u}_n+\mathbf{\Phi} \mathbf{\Delta q};\boldsymbol{\mu})\mathbf{R}(\mathbf{u}_n+\mathbf{\Phi} \mathbf{\Delta q};\boldsymbol{\mu})=\mathbf{0}
    \label{Least Squares projected residual}
\end{equation}
Let us define the residual vector as follows:
\begin{equation}
    \hat{\mathbf{R}}=\mathbf{K}^T\mathbf{R}=\mathbf{0}
\end{equation}
then eq.\ref{Least Squares projected residual} may be written as:
\begin{equation}
    \mathbf{\Phi}^T \hat{\mathbf{R}}(\mathbf{u}_n+\mathbf{\Phi} \mathbf{\Delta q};\boldsymbol{\mu})=\mathbf{0}
    \label{Least Squares projected residual modified}
\end{equation}
which is identical to its Galerkin counterpart in eq.\ref{Galerkin projected residual}, aside from the $\hat{\mathbf{R}}$ operator. In fact, this introduces a crucial difference insofar as hyper-reduction is concerned. Indeed, if eq.\ref{Least Squares projected residual modified} is expressed in terms of elemental contributions:
\begin{equation}
\begin{split}
    \mathbf{\Phi} ^T\mathbf{K}^T\mathbf{R}&=\mathbf{\Phi}^T(\sum_e^M\mathbf{L}^{e^T}\mathbf{K}^{e^T}\mathbf{L}^{e})\mathbf{R}\\
    & = (\sum_h^M(\mathbf{L}^{e}\mathbf{\Phi})^T\mathbf{K}^{e^T}\mathbf{L}^{e})\mathbf{R}\\
    & = (\sum_h^M\mathbf{\Phi}^{e^T}\mathbf{K}^{e^T}\mathbf{L}^{e})\mathbf{R}\\
    \label{Leasts Squares Projected Residuals}
\end{split}
\end{equation}
Let us define now the element quantity:
\begin{equation}
    \tilde{\mathbf{R}}^e:=\mathbf{L}^e\mathbf{R}
    \label{Assembled residual vector}
\end{equation}
These are the entries of the \textit{assembled residual vector} corresponding to the DOFs of element $e$, not to be confused with $\mathbf{R}^e$, which is the contribution of element $e$ to the residual (before assembly).\\ \\
In consequence:
\begin{equation}
    \sum_e^M\mathbf{\Phi}^{e^T}\hat{\mathbf{R}}^e(\mathbf{u}_n+\mathbf{\Phi} \mathbf{\Delta q};\boldsymbol{\mu})=\mathbf{0}
\end{equation}
where:
\begin{equation}
    \hat{\mathbf{R}}^e:=\mathbf{K}^{e^T}\tilde{\mathbf{R}}^e
\end{equation}
The key difference is that the computation of each element contribution $\hat{\mathbf{R}}^e$ requires the determination of the residual vectors of all the elements sharing nodes with element $e$ (patch of elements), this is deduced from eq.\ref{Assembled residual vector}, and it is sketched in figure \ref{fig:Patch of elements associated to a selected element of a 2D and 3D mesh.}. With a LSPG scheme, this results in the need to include the neighbors of each mesh entity \cite{Grimberg2021}, which forces a complementary mesh based on the patch of elements for a given set of elements $\mathbf{Z}\subset \{1,2,\hdots,M\}$. This being independent of the element selection method.

This peculiarity of problems arising from minimization of residuals suggests adjusting the ECM search process in such a way that, once a particular element is selected, the patches associated with it are used as candidates for the next step in the algorithm (to maximize the overlap between the patches). Even if we can use the hyper reduction scheme described in Section \ref{Galerkin-based ROMs} for the Galerkin method, the number of elements to consider in the finite element analyses will always be greater than in the Galerkin case. 
\begin{figure}[H]
\centering
\fbox{\includegraphics[width=0.5\linewidth]{Images/LSPG_HROM/Patch_2D_3D.png}}
\caption{Patch of elements associated to a selected element of a 2D and 3D mesh. (a) 2D, (b) 3D. Red: Patch of elements, Blue: Selected element}
\label{fig:Patch of elements associated to a selected element of a 2D and 3D mesh.}
\end{figure}
